Interactive Decision Making for Autonomous Vehicles in Dense Traffic

Dense urban traffic environments can produce situations where accurate prediction and dynamic models are insufficient for successful autonomous vehicle motion planning. We investigate how an autonomous agent can safely negotiate with other traffic participants, enabling the agent to handle potential deadlocks. Specifically we consider merges where the gap between cars is smaller than the size of the ego vehicle. We propose a game theoretic framework capable of generating and responding to interactive behaviors. Our main contribution is to show how game-tree decision making can be executed by an autonomous vehicle, including approximations and reasoning that make the tree-search computationally tractable. Additionally, to test our model we develop a stochastic rule-based traffic agent capable of generating interactive behaviors that can be used as a benchmark for simulating traffic participants in a crowded merge setting.

==> driving.tex <==
% WHAT'S THE PROBLEM? autonomous driving intersections
\blue{
One of the most challenging problems for autonomous vehicles is to handle unsignaled intersections in urban environments. In order to successfully navigate through an intersection, it is necessary to understand vehicle dynamics, interpret the intent of other drivers, and behave predictably so that other drivers can appropriately respond. Learning this behavior requires optimizing multiple conflicting objectives including safety, efficiency, and minimizing the disruption of traffic. Balancing these trade-offs 
can be challenging even for human drivers: 20\% of all accidents occur at intersections \cite{Statistics2014}. Acquiring the ability to perform optimally at traffic junctions can both extend the abilities of autonomous agents and increase safety through driver assistance when a human driver is in control.

% WHAT HAVE OTHERS DONE? darpa, hierarchical state machines, pomcps, ttc

A number of rule-based strategies have already been applied to intersection handling, including  cooperative \cite{hafner2013cooperative} and heuristic \cite{alonso2011autonomous} approaches. Cooperative approaches require vehicle-to-vehicle communication and thus not scalable to general intersection handling. The current state of the art is a rule-based method based on time-to-collision (TTC) \cite{minderhoud2001extended, van1993time}, which is a widely used heuristic as a safety indicator in the automotive industry \cite{vogel2003comparison}. Variants of the TTC approach has been used for autonomous driving \cite{ferguson2008reasoning} and the DARPA urban challenge, where hand engineered hierarchical state machines were a popular approach to handle intersections \cite{darpa2, urmson2008autonomous}. TTC is currently the method we employ on our autonomous vehicle \cite{cosgun2017towards}.

While TTC has many benefits - it is relatively reliable, generates behavior that is easy to interpret, and can be tuned to reach a high level of safety - it also has limitations. First, the TTC models assume constant velocity, which ignores nearly all information concerning driver intent. This is problematic: in the DARPA Urban Challenge, one reason behind a collision between two autonomous cars was ``failure to anticipate vehicle intent'' \cite{darpa1}. Second, in public roads the often unpredictable behavior of human drivers complicates the use of rule-based algorithms. Third, in many cases an agent using TTC may be overly cautious, creating unnecessary delays. These reasons motivate our investigation of machine-learning based approaches for intersection handling in autonomous vehicles.
}
\begin{figure}[t]
\centering
  \includegraphics[width=0.48\textwidth]{images/intro.pdf}
  %\includegraphics[scale=1.0]{figurefile}
  \caption{Crossing a busy intersection. Red car is the autonomous vehicle and yellow cars are oncoming traffic. The objective is to determine the acceleration profile along the path.}
  \label{fig:sumo}
  \vspace{-0.2cm}
\end{figure}
\blue{
A number of machine learning based approaches have been used for the intersection handling, such as imitation learning, online planning and offline learning. In imitation learning, the policy is learned from a human drivers \cite{bojarski2016end}, however  this policy does not offer a solution if the agent finds itself in a state that is not part of the training data. Online planners compute the best action to take by simulating the future states from the current time step. Online planners based on partially observable Monte Carlo Planning (POMCP) have been shown to handle intersections \cite{bouton2017belief}, but rely on the existence of an accurate generative model. Offline learning tackles the intersection problem, often by using Markov Decision Processes (MDP) in the back-end \cite{song2016intention,brechtel2014probabilistic}. 

In this paper, we use an offline learning method based on Deep Reinforcement Learning (Deep RL), which to our knowledge hasn't previously been studied for the intersection problem. Given the recent success of Deep Learning on a variety of control problems,
\cite{mnih2013playing,levine2016learning,levine2016end} we are interested in evaluating the effectiveness of Deep RL in the domain of intersection handling. As seen in Figure \ref{fig:sumo}, the autonomous vehicle is at an unsignaled intersection where the traffic is flowing in both directions. The autonomous vehicle starts from an initially stopped position. The path is assumed to be given by a higher level process, and the proposed approach is tasked to determine the acceleration profile along the path.

%Can we learn a better controller? (DQN contribution) 
The contributions of this paper are three-fold. The first contribution is the novel way we combine several recent deep learning techniques in order to boost learning speed and improve performance. We use dynamic frame skipping \cite{srinivas2017dynamic} to expedite the system learning repeated actions, and prioritized reply \cite{schaul2015prioritized} to ensure the network balances learning both positive and negative cases. Additionally, we take advantage of the off-policy nature imposed by experience replay learning to calculate and train on the full n-step return \cite{peng1996incremental} which we found greatly reduces the learning time of DQNs.

%What are the limitations of each approach? (Analysis contribution)

The second contribution is our analysis of how well the DQN performs as compared to TTC in five different intersection simulation scenarios, considering safety metrics such as collision rate, and efficiency metrics such as success rate, total time to complete the intersection, and disruption of traffic. We further offer insight on the types of scenarios where DQN could be preferable over TTC. This analysis is of interest beyond the specific choice of DQNs as a base learner as it identifies scenarios where TTC can be improved and suggests methods that could improve it.


%How generalizable is that controller? (Transfer contribution) 

The third contribution is the analysis on how well the trained DQN policies transfer to different scenarios. To ensure safety and reliability, any learning system must generalize well to out-of-sample data. To fully appreciate the strengths and failings of our learned networks we run each network on intersection scenarios it did not train on. This analysis allows us to identify when we can and cannot expect a network to succeed in novel situations.

The rest of the paper is organized as follows: In Chapter \ref{sec:approach} we describe the DQN formulation. In Chapter \ref{sec:experiments}, we describe the experimental setup and simulation environment. In Chapter \ref{sec:results} we discuss the TTC and DQN results, and investigate how DQN policies transfer to different scenarios. In Chapter \ref{sec:conclusion}, we draw our conclusions pertaining this work.
}

%%%%%

\subsection{State-Action Representations}
\blue{
Autonomous vehicles use a suite of sensors, and allow for planning at multiple levels of abstraction. This allows for a wide variety of state and action representations. An exploratory search of representations showed the selection of the representation had a significant impact on the agent's ability to learn. In this paper we present the two representations we found to work well.

\noindent \textbf{Time-to-Go}
In the Time-to-Go representation the desired path is provided to the agent and the agent determines the timing of departure through a sequences of actions to wait or go. Every \emph{wait} action is followed by another wait or go decision, meaning every trajectory is a series of wait decisions terminating in a go decision, and the agent is not allowed to wait after the go action has been selected.

A birds eye view of space is discretized into a grid in Cartesian coordinates. Every car in the space is represented by it's heading angle, velocity, and bias term.  

The sequential scenario allows for more complex behaviors: the agent could potential slow down half way through the intersection and wait for on coming traffic to pass. The Time-to-Go representation more closely compares to TTC, placing importance on the time of departure.
By analyzing the sequential action representation we are able to observe if their is a benefit to allowing more complex behaviors. The Time-to-Go representation focuses on the departure time, allowing us to specifically probe how changes in departure time can affect performance. 
}


% We evaluate each method according to four metrics and run 10,000 trials of each scenario in order to collect our statistics. The metrics are as follows:
% \begin{itemize}
% \item \textbf{Percentage of successes:} the percentage of the runs the car successfully reached the goal. This metric takes into both collisions and time-outs.
% \item \textbf{Percentage of collisions:} a measure of the safety of the method. 
% \item \textbf{Average time:} how long it takes a successful trial to run to completion.
% \item \textbf{Average braking time:} the amount of time other cars in the simulator are braking, this can be seen as a measure of how disruptive the autonomous car is to traffic.
% \end{itemize}
% }
